CERES: Pretraining of Graph-Conditioned Transformer for Semi-Structured Session Data

User sessions empower many search and recommendation tasks on a daily basis. Such session data are semi-structured, which encode heterogeneous relations between queries and products, and each item is described by the unstructured text. Despite recent advances in self-supervised learning for text or graphs, there lack of self-supervised learning models that can effectively capture both intra-item semantics and inter-item interactions for semi-structured sessions. To fill this gap, we propose CERES, a graph-based transformer model for semi-structured session data. CERES learns representations that capture both inter- and intra-item semantics with (1) a graph-conditioned masked language pretraining task that jointly learns from item text and item-item relations; and (2) a graph-conditioned transformer architecture that propagates inter-item contexts to item-level representations. We pretrained CERES using ~468 million Amazon sessions and find that CERES outperforms strong pretraining baselines by up to 9% in three session search and entity linking tasks.

==> downstream.tex <==

% \subsection{Downstream Tasks}
% We report experiment results in three common applications in online e-commerce platforms that could benefit from session information:
% \begin{itemize}
%     \item Semantic product search. Given a customer's session, retrieve the product that the customer is most likely to purchase.
%     \item Semantic query search. Given a customer's session up to a certain time, predict what the customer might be interested in searching next.
%     \item Entity linking. Given a customer's session, link the attributes of products that the customer is most likely to be interested in.
% \end{itemize}

\section{Main Results}

\zc{Your presented results are scarce. Where are the results for varying training sizes?
  Where are case studies or visualization?}

\input{exp_pr}
\input{exp_qr}
\input{exp_el}

\subsection{Ablation Studies}

\begin{table}[h]
    \centering
    \begin{tabular}{c|cc}
       Method  &  Recall@100 & MAP@1100 \\
       Bert &  88.25 & 25.69 \\
       Roberta & 89.25 & 27.57 \\
       Product Bert & 97.188 & 30.872 \\
       SQSP Bert & 98.601 & 31.348 \\
       Congrats & 84.280 & 32.522 
    \end{tabular}
    \caption{Experiment results on Product Search without session information. In this experiment, only last queries of sessions are used to retrieve products for each session.  }
    \label{tab:experiments_wo_session}
\end{table}

In this section, we perform ablation experiments over a number of aspects of our proposed model in order to better understand performance improvement relative to baselines.
\rui{In this part we frequently need to refer to graph neural networks and conditional transformers as a whole. I call it Graph Encoding Modules now but will change later.}

\subsubsection{Effects of Graph Encoding Modules in Finetuning}
We demonstrate the importance of graph encoding modules, i.e. the graph neural networks and the conditional transformer. We follow the exactly same finetuning setting and report results of \emph{Congrats w/o Cond}. Specifically, in Congrats w/o Cond, we take the output embeddings of the backbone transformer of Congrats of objects in sessions and take average pooling as the session embedding. Basically, we use the backbone transformer of Congrats essentially in the same manner as Bert or Product Bert, etc. In this approach, information in the whole session are still known to the model. However, the specifically designed modules for session graphs were not involved in the forward computation.

Results are shown in Table~\ref{tab:exp_results1}.
In product search and entity linking, the performance of Congrats w/o Cond is comparable with Congrats, showing minor drops in performance when the cutoff for evaluation metrics are high. 
In query search, the performance drop accross all metrics are more significant, approaching about 5\%. 
In all three experiments, Congrats w/o Cond still outperforms baseline models
with a significant advantage. \zc{move the results from table 2 to here, use bar
plots}

These experiment results show that the graph encoding modules bring performance improvement consistently across all tasks in the finetuning stage and especially in the pretraining stage. 
Recall that the backbone of our Congrats model is trained with almost the same corpus with the baseline models: Product Bert has access to product informations, SQSP Bert has access to queries and product informations, the same as Congrats backbone. 
The improvement of Congrats w/o Cond can be attribtued to the more efficient exploitation of session structrues in the pretraining stage made possible by the session graph representation, the graph encoding modules, and the conditioned masked language modeling strategy, and the knowledge of session structures can be transferred to finetuning stage without these modules.
In practice, it could be desirable to use Congrats w/o Cond in favor of Congrats for efficiency considerations without fear of drastic drop in the ability to utilize session information.

\subsubsection{Effects of Pretraining on Graph Encoding Modules}
In this section, we ascertain if pretraining on graph encoding modules is helpful. Indeed, one might directly attach graph neural networks and the conditional transformer after a pretrained language model, such as Bert or Product Bert, without pretraining on them. We 
\rui{I added this recently. Need to add some experiments}

\subsubsection{Effects of GNN Modules in Pretraining}
We've also pretrained a version of our model without GNN layers, as shown as \emph{Congrats w/o GNN} in Table\ref{tab:exp_results1}. 
Specifically, it follow the same pretraining settings as Congrats. However, instead of using GNN to aggregate session information for each node, 
it directly uses the pooled embedding of the backbone transformer output as node embeddings. These node embeddings are then directly used as condition tokens for conditional masked language modeling. 

Results are shown in Table~\ref{tab:exp_results1}. Across all tasks and metrics, Congrats w/o GNN observes about 1\%-2\% performance drop. 
It shows that GNN is helpful to capture the interactions between nodes in session graphs as well as obtaining session embeddings with richer information. 


\subsubsection{Effects of Session Information}

In practice, sometimes session information is not available. In such cases, we could only infer the intent of customers by single queries. 
In this experiment, instead of averaging embeddings for objects in sessions, we use only the embedding of the last queries in the session graph for inference. The rest of the experiment setting is the same. 

 Table~\ref{tab:experiments_wo_session} shows experiment results. Performance for all baselines dropped significantly compared with scores in Table~\ref{tab:exp_results1}, especially in terms of MAP.  
 The advantage of our model is not as significant as in previous settings, but our model still remains competitive, achieving the highest MAP@100 at the cost of reduced Recall@100.


\subsubsection{Feature-based Approaches}
\rui{I added this session recently. Will add experiments later}

==> exp_1_tabular.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
=\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrrrrl}
\cline{1-12}
Task                                                                       & Method            & \multicolumn{1}{l}{map@1} & \multicolumn{1}{l}{recall@1} & \multicolumn{1}{l}{mapq@1} & \multicolumn{1}{l}{map@32} & \multicolumn{1}{l}{recall@32} & \multicolumn{1}{l}{mapq@32} & \multicolumn{1}{l}{map@64} & \multicolumn{1}{l}{recall@64} & \multicolumn{1}{l}{mapq@64} & \multicolumn{1}{l}{} &                      \\ \cline{1-12}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Product \\ Search\end{tabular}} & Bert              & 79.808                    & 79.749                       & 80.769                     & 83.625                     & 94.959                        & 84.176                      & 83.652                     & 96.27                         & 84.118                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 81.25                     & 81.308                       & 82.168                     & 86.622                     & 98.864                        & 87.278                      & 86.63                      & 99.126                        & 87.243                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Electra           & 71.955                    & 72.13                        & 73.427                     & 79.609                     & 97.771                        & 80.596                      & 79.638                     & 99.038                        & 80.545                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Product Bert      & 81.09                     & 81.571                       & 82.867                     & 87.622                     & 99.563                        & 88.62                       & 87.622                     & 99.563                        & 88.62                       &                      & \multicolumn{1}{r}{} \\
                                                                           & SQSP Bert         & 73.237                    & 73.383                       & 74.126                     & 81.635                     & 97.99                         & 82.372                      & 81.654                     & 98.951                        & 82.349                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats          & 89.103                    & 89.612                       & 90.559                     & 92.852                     & 99.155                        & 93.819                      & 92.852                     & 99.155                        & 93.819                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats w/o Cond & 89.423                    & 89.729                       & 90.559                     & 92.135                     & 98.339                        & 92.88                       & 92.151                     & 99.038                        & 92.898                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats w/o GNN  & 88.744                    & 89.166                       & 90.084                     & 92.067                     & 97.98                         & 92.865                      & 92.075                     & 98.33                         & 92.873                      &                      & \multicolumn{1}{r}{} \\ \cline{1-11}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Query \\ Search\end{tabular}}   & Bert              & 45.353                    & 45.526                       & 45.827                     & 59.604                     & 94.19                         & 59.942                      & 59.661                     & 96.809                        & 60.001                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 45.032                    & 44.981                       & 45.499                     & 57.145                     & 89.525                        & 57.386                      & 57.226                     & 93.29                         & 57.468                      &                      &                      \\
                                                                           & Electra           & \multicolumn{1}{l}{NA}    & \multicolumn{1}{l}{NA}       & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{} &                      \\
                                                                           & Product Bert      & 49.679                    & 49.73                        & 50                         & 62.935                     & 94.185                        & 64.726                      & 62.97                      & 95.594                        & 64.618                      &                      &                      \\
                                                                           & SQSP Bert         & 41.667                    & 42.536                       & 42.626                     & 55.549                     & 93.735                        & 58.027                      & 55.629                     & 96.882                        & 58.094                      &                      &                      \\
                                                                           & Congrats          & 61.538                    & 61.96                        & 62.23                      & 73.7                       & 97.122                        & 75.551                      & 73.724                     & 98.022                        & 75.578                      &                      &                      \\
                                                                           & Congrats w/o Cond & 55.769                    & 56.745                       & 56.835                     & 68.752                     & 95.683                        & 71.145                      & 68.792                     & 97.302                        & 71.19                       &                      &                      \\
                                                                           & Congrats w/o GNN  & 60.737                    & 61.691                       & 61.871                     & 73.424                     & 96.942                        & 75.767                      & 73.437                     & 97.662                        & 75.782                      & \multicolumn{1}{l}{} &                      \\ \cline{1-11}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Entity\\ Linking\end{tabular}}  & Bert              & 13.782                    & 14.397                       & 14.828                     & 19.235                     & 43.779                        & 20.441                      & 19.465                     & 53.822                        & 20.435                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 30.609                    & 30.848                       & 31.897                     & 34.041                     & 49.454                        & 35.324                      & 34.161                     & 55.23                         & 35.432                      &                      &                      \\
                                                                           & Electra           & \multicolumn{1}{l}{NA}    & \multicolumn{1}{l}{NA}       & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{} &                      \\
                                                                           & Product Bert      & 66.827                    & 66.393                       & 66.606                     & 74.611                     & 94.404                        & 75.287                      & 74.641                     & 96.046                        & 75.321                      &                      &                      \\
                                                                           & SQSP Bert         & 65.342                    & 66.453                       & 66.432                     & 75.324                     & 93.586                        & 74.254                      & 74.322                     & 95.5                          & 74.3                        &                      &                      \\
                                                                           & Congrats          & 75.481                    & 75.456                       & 75.547                     & 81.121                     & 95.255                        & 81.787                      & 81.16                      & 96.898                        & 81.832                      &                      &                      \\
                                                                           & Congrats w/o Cond & 75.481                    & 75.456                       & 75.547                     & 81.121                     & 95.255                        & 81.787                      & 81.16                      & 96.898                        & 81.832                      &                      &                      \\
                                                                           & Congrats w/o GNN  & 73.718                    & 72.536                       & 72.628                     & 80.046                     & 93.796                        & 79.743                      & 80.096                     & 95.985                        & 79.799                      & \multicolumn{1}{l}{} & \\       \hline \\
\end{tabular}%
}

==> exp_2_tabular.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
=\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrrrrl}
\cline{1-12}
Task                                                                       & Method            & \multicolumn{1}{l}{map@1} & \multicolumn{1}{l}{recall@1} & \multicolumn{1}{l}{mapq@1} & \multicolumn{1}{l}{map@32} & \multicolumn{1}{l}{recall@32} & \multicolumn{1}{l}{mapq@32} & \multicolumn{1}{l}{map@64} & \multicolumn{1}{l}{recall@64} & \multicolumn{1}{l}{mapq@64} & \multicolumn{1}{l}{} &                      \\ \cline{1-12}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Product \\ Search\end{tabular}} & Bert              & 79.808                    & 79.749                       & 80.769                     & 83.625                     & 94.959                        & 84.176                      & 83.652                     & 96.27                         & 84.118                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 81.25                     & 81.308                       & 82.168                     & 86.622                     & 98.864                        & 87.278                      & 86.63                      & 99.126                        & 87.243                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Electra           & 71.955                    & 72.13                        & 73.427                     & 79.609                     & 97.771                        & 80.596                      & 79.638                     & 99.038                        & 80.545                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Product Bert      & 81.09                     & 81.571                       & 82.867                     & 87.622                     & 99.563                        & 88.62                       & 87.622                     & 99.563                        & 88.62                       &                      & \multicolumn{1}{r}{} \\
                                                                           & SQSP Bert         & 73.237                    & 73.383                       & 74.126                     & 81.635                     & 97.99                         & 82.372                      & 81.654                     & 98.951                        & 82.349                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats          & 89.103                    & 89.612                       & 90.559                     & 92.852                     & 99.155                        & 93.819                      & 92.852                     & 99.155                        & 93.819                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats w/o Cond & 89.423                    & 89.729                       & 90.559                     & 92.135                     & 98.339                        & 92.88                       & 92.151                     & 99.038                        & 92.898                      &                      & \multicolumn{1}{r}{} \\
                                                                           & Congrats w/o GNN  & 88.744                    & 89.166                       & 90.084                     & 92.067                     & 97.98                         & 92.865                      & 92.075                     & 98.33                         & 92.873                      &                      & \multicolumn{1}{r}{} \\ \cline{1-11}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Query \\ Search\end{tabular}}   & Bert              & 45.353                    & 45.526                       & 45.827                     & 59.604                     & 94.19                         & 59.942                      & 59.661                     & 96.809                        & 60.001                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 45.032                    & 44.981                       & 45.499                     & 57.145                     & 89.525                        & 57.386                      & 57.226                     & 93.29                         & 57.468                      &                      &                      \\
                                                                           & Electra           & \multicolumn{1}{l}{NA}    & \multicolumn{1}{l}{NA}       & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{} &                      \\
                                                                           & Product Bert      & 49.679                    & 49.73                        & 50                         & 62.935                     & 94.185                        & 64.726                      & 62.97                      & 95.594                        & 64.618                      &                      &                      \\
                                                                           & SQSP Bert         & 41.667                    & 42.536                       & 42.626                     & 55.549                     & 93.735                        & 58.027                      & 55.629                     & 96.882                        & 58.094                      &                      &                      \\
                                                                           & Congrats          & 61.538                    & 61.96                        & 62.23                      & 73.7                       & 97.122                        & 75.551                      & 73.724                     & 98.022                        & 75.578                      &                      &                      \\
                                                                           & Congrats w/o Cond & 55.769                    & 56.745                       & 56.835                     & 68.752                     & 95.683                        & 71.145                      & 68.792                     & 97.302                        & 71.19                       &                      &                      \\
                                                                           & Congrats w/o GNN  & 60.737                    & 61.691                       & 61.871                     & 73.424                     & 96.942                        & 75.767                      & 73.437                     & 97.662                        & 75.782                      & \multicolumn{1}{l}{} &                      \\ \cline{1-11}
\multirow{8}{*}{\begin{tabular}[c]{@{}l@{}}Entity\\ Linking\end{tabular}}  & Bert              & 13.782                    & 14.397                       & 14.828                     & 19.235                     & 43.779                        & 20.441                      & 19.465                     & 53.822                        & 20.435                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           & 30.609                    & 30.848                       & 31.897                     & 34.041                     & 49.454                        & 35.324                      & 34.161                     & 55.23                         & 35.432                      &                      &                      \\
                                                                           & Electra           & \multicolumn{1}{l}{NA}    & \multicolumn{1}{l}{NA}       & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{NA}     & \multicolumn{1}{l}{NA}        & \multicolumn{1}{l}{NA}      & \multicolumn{1}{l}{} &                      \\
                                                                           & Product Bert      & 66.827                    & 66.393                       & 66.606                     & 74.611                     & 94.404                        & 75.287                      & 74.641                     & 96.046                        & 75.321                      &                      &                      \\
                                                                           & SQSP Bert         & 65.342                    & 66.453                       & 66.432                     & 75.324                     & 93.586                        & 74.254                      & 74.322                     & 95.5                          & 74.3                        &                      &                      \\
                                                                           & Congrats          & 75.481                    & 75.456                       & 75.547                     & 81.121                     & 95.255                        & 81.787                      & 81.16                      & 96.898                        & 81.832                      &                      &                      \\
                                                                           & Congrats w/o Cond & 75.481                    & 75.456                       & 75.547                     & 81.121                     & 95.255                        & 81.787                      & 81.16                      & 96.898                        & 81.832                      &                      &                      \\
                                                                           & Congrats w/o GNN  & 73.718                    & 72.536                       & 72.628                     & 80.046                     & 93.796                        & 79.743                      & 80.096                     & 95.985                        & 79.799                      & \multicolumn{1}{l}{} &                      \\
\multirow{9}{*}{}                                                          &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{l}{} &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           &                   & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{} &                     
\end{tabular}%
}

==> exp_3_tabular.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrrrrrrrrrrl}
\cline{1-12}
Task &
  Method &
  \multicolumn{1}{l}{map@1} &
  \multicolumn{1}{l}{recall@1} &
  \multicolumn{1}{l}{mapq@1} &
  \multicolumn{1}{l}{map@32} &
  \multicolumn{1}{l}{recall@32} &
  \multicolumn{1}{l}{mapq@32} &
  \multicolumn{1}{l}{map@64} &
  \multicolumn{1}{l}{recall@64} &
  \multicolumn{1}{l}{mapq@64} &
  \multicolumn{1}{l}{} &
   \\ \cline{1-12}
   
   \multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Entity\\ Linking\end{tabular}}  & Bert              & 12.66                     & 12.105                       & 12.226                     & 18.081                     & 38.96                         & 18.152                      & 18.298                     & 49.179                        & 18.399                      & \multicolumn{1}{l}{} &                      \\
                                                                           & Roberta           &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           & Electra           & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{} &                      \\
                                                                           & Product Bert      & 66.827                    & 66.393                       & 66.606                     & 74.611                     & 94.404                        & 75.287                      & 74.641                     & 96.046                        & 75.321                      &                      &                      \\
                                                                           & SQSP Bert         & 65.342                    & 66.453                       & 66.432                     & 75.324                     & 93.586                        & 74.254                      & 74.322                     & 95.5                          & 74.3                        &                      &                      \\
                                                                           & Congrats          & 70.673                    & 69.86                        & 70.073                     & 76.6                       & 90.146                        & 76.625                      & 76.646                     & 92.336                        & 76.677                      &                      &                      \\
                                                                           & Congrats w/o Cond &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      &                      \\
                                                                           & Congrats w/o GNN  & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{} &                      \\
                                                                                   
\
\end{tabular}}

==> exp_data.tex <==


\vpara{Finetuning.}
In downstream tasks, the models are asked to predict or recommend properties relevant to the purchased product or the last query where the customer made the last purchase.
Hence, it is imperative to make sure such information are not leaked in the finetuning stage. 
Specifically,
we collected a week's sessions from September 1 2020 to September 7 2020, a different period from where the data used in pretraining are collected, to make sure that sessions in pretraining and finetuning stages are non-overlapping. 
We sample training, validation, and testing sets from the collected sessions. 
To make sure the evaluation is nontrivial, the last queries of sessions from the testing set are disjoint from those from the training and validation set, so that the models cannot rely simply on the superficial clue by the last query. 
We make the following two datasets: 
\begin{enumerate}
    \item Sessions-without-purchase. In these sessions, final purchase action and the purchased product information are removed from the session. If the purchased product were viewed or interacted with by the customer in the same session, these are removed as well.
    \item Sessions-without-last-query. In these sessions, the final purchase actions are removed as just described. In addition, the last queries where the customer made the purchases were removed as well, as well as their previous occurrences. 
\end{enumerate}
The first dataset completely removed the information of the last purchase from the session so that recommendations to the customers about purchases can be make. The second dataset further removes the last queries, so that it is possble to recommend them the next search action. 

\subsection{Evaluation Metrics}
Our downstream tasks can all be formulated as recommendation tasks. 
Hence, we propose to evaluate the effectiveness of models on these tasks with common recommendation metrics: \emph{Mean Average Precision} (MAP), \emph{Mean Reciprocal Rank} (MRR), \emph{Recall}, and \emph{Hit}. 
In addition to directly applying these metrics on sessions which can have at most one relevant item, we consolidate the predictions for sessions with the same last queries before applying these metrics to match the traditional recommendation setting.

\vpara{Mean Average Precision.}
Suppose that for a session, \emph{m} items are relevant and \emph{N} items are retrieved by the model, the \emph{Average Precision} (AP) of a session is defined as 
\begin{equation}
    \mathrm{AP}@\mathrm{N} = \frac{1}{\min(m, N)}\sum_{k=1}^N P(k) rel(k)
\end{equation},
where \(P(k)\) is the precision of the top \emph{k} retrieved items, and \(rel(k)\) is an indicator function of whether the \(k\)th item is relevant. 
As we have at most one relevant item for each session, the above metric reduces to \( \frac{1}{r} \), where \(r\) is the rank of the relevant item in the retrieved list, and \(k=\infty\) when the relevant item is not retrieved. MAP@N averages AP@N over all sessions,
\begin{equation}
    \mathrm{MAP}@\mathrm{N} = \frac{1}{|\mathcal{S}|}\sum_{s\in\mathcal{S}} \frac{1}{r_s}
\end{equation}
where \(r_s\) is the rank of the relevant item for a specific session \(s\). MAP in this case is equivalent to MRR.

\vpara{Mean Average Precision by Queries (MAPQ).}
Different from MAP, MAPQ averages AP over last queries instead of sessions. 

\vpara{Mean Reciprocal Rank by Queries (MRRQ).}

\vpara{Recall.}

\vpara{Hit by Query.}

==> exp_el.tex <==
\subsection{Entity Linking}

The task of entity linking involves assigning a search session the designed attributes of potential products that the customers intent to purchase.
Entity linking is also similar to a traditional multi-class classification task. However, the size of potential attribute space (label space) is so large that most attributes have only a few occurrences in the entire dataset. 
Furthermore, 
with the help of session context, it is naturally easier to infer what attributes of products the customers are looking for.


In Table~\ref{tab:exp_results1} we report the experiment results on entity linking.
In this task, it can be seen that domain-specific pretraining plays an vital role to satisfactory performance.
Specifically, for pretrained models trained on general domain, such as Bert, Roberta, and Electra, the performance gap between them and other models such as Product Bert are larger than the rest of the tasks. This shows that domain-specific knowlegde is vital in finding the relation between queries, products, and attributes.

==> exp_pr.tex <==
\subsection{Semantic Product Search}

\chen{When we introduce the customer session data, we need to mention the data is cleaned and anonymized.}

In semantic product search, given customer generated search queries, it is desired to retrieve the most relevant products that customers are interested in.
Sessions are naturally a crucial piece of information for product search, as we could assume that in most cases, the past behavioral information in a session, i.e. past search queries and viewed products, is relevant to the actual product that the customers are interested in. 
Hence, it is natural to expect that our pretrained model can improve performance on semantic product search.


Table~\ref{tab:exp_results1} shows the experiment results. It can be shown that our model outperforms baseline models by 6\% in MAP@1. 
All these models have access to the information in the entire session. 
Specifically, 
traditional language models perform similarly. Although they do have access to session information, such information are not utilized efficiently, which is crucial to their performance.


==> exp_qr.tex <==
\subsection{Semantic Query Search}
In semantic query search, we seek to predict the query that are most relevant to customers intent.
The relevancy between queries and customer intents are determined by whether the customers have made purchases on products returned by search results by the queries. In a similar manner to semantic product search, session information is crucial to understanding customer intent in a specific search session. As sessions help understanding the intent of customers on purchasing products, they naturally could help with providing the most helpful queries to lead to a purchase.

Table~\ref{tab:exp_results1} shows the experiment results on query recommendation as well. 
It can be seen that our model can improve performance over baseline by over 10\%. 

==> exp_results_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h]
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\input{exp_1_tabular}
\caption{Experiment results. All baseline methods adopt the same retrieval head and are finetuned according to Section~\ref{sec:finetuning}.
All of the models will consider all information in the input session, where traditional language models take the average pool of objects in a session, and Congrats utilizes a pretrained graph encoder and conditioned language model modules. \zc{use separate tables/figures for the three different tasks.}Particularly, Congrats w/o Cond is Congrats finetuned without the conditional transformer and GNN layers, and Congrats w/o GNN is Congrats model pretrained without GNN layers. 
\emph{NA} in the table means that the method was not able to produce a
prediction better than random guessing.}

\label{tab:exp_results1}
\end{table*}


==> exp_results_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h ]
\begin{tabular}{llrrrrrrrrrl}
Task                                                                               & Method            & \multicolumn{1}{l}{map@1} & \multicolumn{1}{l}{recall@1} & \multicolumn{1}{l}{mapq@1} & \multicolumn{1}{l}{map@32} & \multicolumn{1}{l}{recall@32} & \multicolumn{1}{l}{mapq@32} & \multicolumn{1}{l}{map@64} & \multicolumn{1}{l}{recall@64} & \multicolumn{1}{l}{mapq@64} &                      \\
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Query \\ Recommendation\end{tabular}}   & Bert              &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Roberta           &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Product Bert      & 49.679                    & 49.73                        & 50                         & 62.935                     & 94.185                        & 64.726                      & 62.97                      & 95.594                        & 64.618                      &                      \\
                                                                                   & SQSP Bert         & 41.667                    & 42.536                       & 42.626                     & 55.549                     & 93.735                        & 58.027                      & 55.629                     & 96.882                        & 58.094                      &                      \\
                                                                                   & Session Bert      &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Congrats          & 60.096                    & 60.881                       & 61.151                     & 72.589                     & 97.032                        & 74.767                      & 72.616                     & 98.112                        & 74.701                      &                      \\
                                                                                   & Congrats w/o Cond &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Congrats w/o GNN  & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                      \\
                                                                                   & Congrats w/o SP   & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                      \\
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Product \\ Recommendation\end{tabular}} & Bert              &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Roberta           &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{r}{} \\
                                                                                   & Product Bert      & 81.09                     & 81.571                       & 82.867                     & 87.622                     & 99.563                        & 88.62                       & 87.622                     & 99.563                        & 88.62                       & \multicolumn{1}{r}{} \\
                                                                                   & SQSP Bert         & 73.237                    & 73.383                       & 74.126                     & 81.635                     & 97.99                         & 82.372                      & 81.654                     & 98.951                        & 82.349                      & \multicolumn{1}{r}{} \\
                                                                                   & Session Bert      &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{r}{} \\
                                                                                   & Congrats          & 86.859                    & 87.382                       & 88.516                     & 91.591                     & 99.882                        & 92.655                      & 91.591                     & 99.882                        & 92.655                      & \multicolumn{1}{r}{} \\
                                                                                   & Congrats w/o Cond &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{r}{} \\
                                                                                   & Congrats w/o GNN  & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                      \\
                                                                                   & Congrats w/o SP   & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                      \\
\multirow{9}{*}{\begin{tabular}[c]{@{}l@{}}Entity\\ Linking\end{tabular}}          & Bert              &                           &                              &                            &                            &                               &                             &                            &                               &                             &                      \\
                                                                                   & Roberta           &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{r}{} \\
                                                                                   & Product Bert      & 66.827                    & 66.393                       & 66.606                     & 74.611                     & 94.404                        & 75.287                      & 74.641                     & 96.046                        & 75.321                      & \multicolumn{1}{r}{} \\
                                                                                   & SQSP Bert         & 65.342                    & 66.453                       & 66.432                     & 75.324                     & 93.586                        & 74.254                      & 74.322                     & 95.5                          & 74.3                        & \multicolumn{1}{r}{} \\
                                                                                   & Session Bert      & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{r}{} \\
                                                                                   & Congrats          & 70.673                    & 69.86                        & 70.073                     & 76.6                       & 90.146                        & 76.625                      & 76.646                     & 92.336                        & 76.677                      & \multicolumn{1}{r}{} \\
                                                                                   & Congrats w/o Cond &                           &                              &                            &                            &                               &                             &                            &                               &                             & \multicolumn{1}{r}{} \\
                                                                                   & Congrats w/o GNN  & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                      \\
                                                                                   & Congrats w/o SP   & \multicolumn{1}{l}{}      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}        &                     
\end{tabular}
\end{table*}

==> exp_training.tex <==
\subsection{Pretraining}



==> experiment.tex <==
\section{Experiments}
\label{sec:exp}
\subsection{Experiment Setup}
\label{sec:exp_setup}

In this section we introduce our experiment setup.
Concretely, first we introduce how session data are collected and converted to session graphs.
Then, we introduce how the model is trained.
\zc{you use two pages to describe experiments setup? Why make the setup as a section?}

\subsubsection{Data Collection}

\rui{could need to explain why we use our data, not public. Public lack session information. Our data is also much more difficult and noisy.}
We collected customer sessions from August 1 2020 to August 31 2020 from an online e-commerce platform. 
For every purchase action by any customer, we collect all actions of the same customer before the purchase in the last 600 seconds after the customer activity started or the last purchase as a session. As such, each session is guaranteed to have one and only one purchase at the end of the session. In total, we have collected 468,199,822 sessions. 
%The collected sessions have an average of  actions,    queries, and    interested products.

Each session is associated with at least one products the customer has purchased, viewed, or added to cart. All products that appeared in the said sessions are gathered with their product title, bullet description, and various other attributes. In total, we have 37,580,637 products. 
\hide{
A \emph{session} of a customer is defined as the sequences of actions that customers take before actual purchases. 
Before an actual purchase, the behavioral data of a customer on an e-commerce platform provides informative context for the customer's intent or purchase behavior. 
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{assets/session_graph.pdf}
    \caption{An illustration of example session graph. In this example, the customer produced three queries in sequence, "Harry", "Harry Potter", and "Harry Potter DVD". In the first search attempt, the customer was recommended razor products. In the second and the third attempt, the customer refines query keywords and finally purchased the desired product.}
    \label{fig:session_graph}
\end{figure}
To capture such information, we propose Session Graphs. A shopping \emph{session} is defined as a collection of customer behaviors before the purchase of a product. It includes the customer's actions, queries, the products that the customers clicked on and viewed, and the final purchase of a product. 
To better encode the relational structure within a session, we propose to use
graphs to represent sessions.
}

\subsubsection{Customer Actions}
In a session, customers may perform the following actions:
\zc{this is so specific, use math notations to describe your problem}
\begin{enumerate}
    \item \emph{Search}. The customer prompts the search engine with query keywords, and the search engine returns relevant products. 
    \item \emph{Click}. Given the products returned by the search engine, the custmer clicks on one of them to access the product information.
    \item \emph{Add to Cart}. The customer adds a product to the shopping cart.
    \item \emph{Purchase}. The customer purchases a product.
\end{enumerate}
We call \emph{add to cart} and \emph{purchase} as \emph{transactional actions}. We always assume that \emph{click}, \emph{add to cart} and \emph{purchase} may only happen after a \emph{search}. 

\subsubsection{Session Graph}
\label{sec:session_graph}
We build a graph on the customer-generated actions. Specifically, nodes in this graph are \emph{queries} and \emph{products} that appeared in the session. Queries are generated by search actions, and products are associated with queries via the actions that the customer take after the query. 
Specifically, the following edges are added to the graph to connect queries and products:
\begin{enumerate}
    \item A query is connected to all previous queries the customer generated in this session. The edges are one-directional and are annotated with the distance between queries. 
    \item A query is bidirectionally connected to all products clicked, added to cart, or purchased under this search request. If a customer searches a query and clicked one of the products returned by the search engine, then the query and the product are connected. The edges are annotated with the action type. 
\end{enumerate}
As such, as have a heterogeneous directional graph with different types of nodes and edges. This session graph contains all information of customer actions, queries, products, and their relations in a session. 

\subsubsection{Product Attributes}
A product is represented with a table of attributes. 
\begin{table}
    \begin{tabular}{cl}
        Attribute & Value \\ \hline
        Title & Chemex Pour-over Coffee Maker \\   \hline
        Bullet Description & Just coffee maker. \\ \hline
        Color &  N/A  \\\hline
        Brand & Chemex \\  \hline
        Manufacturer & Chemex \\ \hline
        Product Type & Coffee Maker \\ \hline
    \end{tabular}
    \caption{Example Product Table. Each product is guaranteed to have a title. Most products have bullet descriptions, which can be split into multiple entries. Products could have other attributes, such as color, brand, product type, etc. as well.}
\end{table}
Each product is guaranteed to have a product title and bullet description. In this paper, we regard the product title as the representative sequence of the product, called ``product sequence''. 
A product may have additional attributes, such as product type, color, brand, and manufacturer, depending on specific products.

\subsection{Model Training}
We developed our model based on Megatron-LM~\cite{shoeybi2019megatron}, a BERT-like Transformer framework for large-scale pretraining. We used 768 as the hidden size, a 12-layer transformer blocks as the backbone language model, a two-layer Graph Attention Network and three-layer Transformer as the conditioned language model layers.
The model is trained for 300,000 steps with a batch size of 512 sessions. The parameters are updated with Adam, with peak learning rate as $3e-5$, $1\%$ steps for linear warm-up, and linear learning rate decay after warm-up until the learning rate reaches the minimum $1e-5$.

\input{exp_results_1}

\subsubsection{Training parameters}
For each model, 
we finetune with three options for learning rates: \(5e-5, 2e-5, 5e-6, 5e-7\) and choose the model with the best performance on the validation set to evaluate. 
In each of these settings, we train with 6.5\% warm-up steps and linear learning rate decay of  to minimum learning rate of    . 
For all experiments, we finetuned the models for 10 epochs. 
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\subsubsection{Evaluation Metrics}
Our downstream tasks can all be formulated as recommendation tasks. 
Hence, we propose to evaluate the effectiveness of models on these tasks with common recommendation metrics: \emph{Mean Average Precision} (MAP), \emph{Mean Reciprocal Rank} (MRR), \emph{Recall}, and \emph{Hit}. 
In addition to directly applying these metrics on sessions which can have at most one relevant item, we consolidate the predictions for sessions with the same last queries before applying these metrics to match the traditional recommendation setting.

\paragraph{Mean Average Precision.}
Suppose that for a session, \emph{m} items are relevant and \emph{N} items are retrieved by the model, the \emph{Average Precision} (AP) of a session is defined as 
\begin{equation}
    \mathrm{AP}@\mathrm{N} = \frac{1}{\min(m, N)}\sum_{k=1}^N P(k) \mathrm{rel}(k),
\end{equation}
where \(P(k)\) is the precision of the top \emph{k} retrieved items, and \(rel(k)\) is an indicator function of whether the \(k\)th item is relevant. 
As we have at most one relevant item for each session, the above metric reduces to \( \frac{1}{r} \), where \(r\) is the rank of the relevant item in the retrieved list, and \(k=\infty\) when the relevant item is not retrieved. MAP@N averages AP@N over all sessions,
\begin{equation}
    \mathrm{MAP}@\mathrm{N} = \frac{1}{|\mathcal{S}|}\sum_{s\in\mathcal{S}} \frac{1}{r_s}
\end{equation}
where \(r_s\) is the rank of the relevant item for a specific session \(s\). MAP in this case is equivalent to MRR.

\paragraph{Mean Average Precision by Queries (MAPQ).}
Different from MAP, MAPQ averages AP over last queries instead of sessions. Suppose \(\mathcal{Q}\) is the set of unique last queries, and \(S(q), q\in\mathcal{Q}\) is the set of sessions whose last queries are \(q\), then the average precision for one query \(q\) is 
\begin{equation}
    \mathrm{APQ}@\mathrm{N} =  \frac{1}{\sum_{i=1}^k \mathrm{rel}(k)}\sum_{k=1}^N \min(1, \frac{\sum_{r_s\leq k}\mathrm{rel}(k)}{k})
\end{equation}
then we sum over all queries to obtain MAPQ@N. 

\paragraph{Mean Reciprocal Rank by Queries (MRRQ).}
MRRQ averages MRR over session last queries instead of sessions. 
\begin{equation}
    MRRQ@N =\frac{1}{|\mathcal{Q}|} \sum_{q\in\mathcal{Q}}\max_{s\in S(q)}(r_s)
\end{equation}

\paragraph{Recall.}
Recall@N calculates the percentage of sessions whose relevant items were retrieved among the top N predictions. 


\subsection{Baseline Methods}
We compare our method with various pretraining frameworks. We include the state-of-the-art pretrained language models for discriminative NLP tasks, including BERT, RoBERTa, and ELECTRA. BERT and RoBERTa learns linguistic features mostly through masked language modeling. Instead of training the language model as a generative model, ELECTRA trains it as a discriminative model against masked tokens in text, which are observed to improve its performance.

Besides language models trained on public and general domain, we have also trained models of similar architecture on domain-specific data for comparison. 
Specifically, we trained the following models:
\begin{itemize}
    \item \emph{Product Bert}. It is a BERT-like transformer trained on Product Corpus, a corpus we constructed by extracting all product information from sessions.
    \item \emph{SQSP Bert}. Recall that SQSP stands for single-product single-query. As it suggests, SQSP Bert is trained on a corpus that consists of one-to-one correspondence between queries and products extracted from all sessions. Besides masked language modeling, it is also trained on a contrastive learning objective, where the model is asked to discriminate ground-truth query-product pairs and random query-product pairs. 
\end{itemize}
The pretraining detail of these models is provided in the supplementary materials. 

\input{downstream}


==> introduction_w.tex <==
\section{Introduction}

% \rui{Sessions are important}

User sessions are ubiquitous in online e-commerce stores. An e-commerce
session contains customer interactions with the platform in a continuous time
span. Within one session, the customer can issue multiple queries and take
various actions on the retrieved products for these queries, such as clicking,
adding to cart, and purchasing. For example, a customer may attempt several
queries, browse different products, add or remove multiple candidates to the
shopping cart before making a final purchase decision. Session data reflect
customer preferences and intents, which have been shown important in many
e-commerce applications, \textit{e.g.}, product recommendation
\cite{wu2019sessionrecom,li2017neuralsession,jannach2017recurrent}, query
recommendation~\cite{cucerzan2007querysession}, and query
understanding~\cite{zhang2020bootstrapping,cheng2020end}.

% ~\rui{this is an Amazon-exlusive term; only internal not published references are available. I referred NER which is similar and can be viewed together with entity linking as query understanding. Hence the changed name }. \zc{add one more
%   example, make it three}

% \rui{Session structure: graph on text}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{assets/session-graph.drawio.pdf}
    \caption{Illustration of a customer session. A session consists of two types of items: queries and products. In this session, the customer searched with three query keywords: ``Harry'', ``Harry Potter'', and ``Harry Potter Book'', viewed different types of products retrieved by these queries, and finally purchased a product. At a lower level, each query and product has its own semantics. At a higher level, the interactions between customers, queries, and products encode rich information about customers' preferences.}
    \label{fig:session-graph}
\end{figure}

In this paper, we consider \textit{semi-structured} session data. As
illustrated in Figure \ref{fig:session-graph}, each session is represented by
a heterogeneous relation graph of e-commerce items, which all have
unstructured text descriptions. At the higher level, sessions contain
customer-query-product interactions, such as customer viewing a product, or
re-writing the current query to a new one. These interactions can be
represented by graph edges denoting different item-item relations. At the
lower level, each graph node belongs to two major item types in e-commerce
sessions: (i) user queries described by search keywords, and (ii) products
described by titles, attributes, customer reviews, and other textual
descriptions. %For a
%successful session-based application, it is crucial to 
Our goal is to simultaneously model both the text and
graph aspects to understand customer preferences and intents in a session
context.

% The session data we consider in this paper are \textit{semi-structured}---each
% session is a heterogeneous relation graph of e-commerce items which all have
% unstructured text descriptions. At the higher level, sessions contain
% customer-query-product interactions, such as customer viewing a product, or
% re-writing the current query to a new one. These interactions can be represented
% as a heterogeneous graph specifying the different relations among the items. At
% the lower level, the two major item types in e-commerce sessions are user
% queries and products, both of which contain informative text descriptions.
% Specifically, queries are described by search keywords; and products are
% described by titles, attributes, customer reviews, and other descriptions. For a
% successful session-based application, it is crucial to model both the text and
% graph aspects to understand customer preferences and intents in a session
% context.

% \rui{existing on session-based methods}

% \rui{existing works on text data}

% \zc{hierarchical graph? Or heterogeneous graph? And add citations.}~\rui{it is hierarchial, but i dont think we need to explain it here. i'll just put graph.}
% \rui{revised verision here}

% \zc{this summarization of existing work is not good: 1. Representation
%   learning and deep learning are pretty much the same category; 2. The
%   different categories are not on the same granularity. 3. Ref 27 does not
%   belong to rule mining.}

Despite recent advances in deep learning for session-based search and
recommendation~\cite{rendle2010factorizing,liu2018stamp,wang2018attention,you2019hierarchical},
it remains an open challenge to model the complex semi-structured session
data: (1) First, existing works on learning from session data usually treat a
session as a sequence or a
graph~\cite{xu2019graph,you2019hierarchical,qiu2020exploiting}. Various models
have been proposed to capture the sequence or graph structure, such as Hidden
Markov Model~\cite{ludewig2019performance,rendle2010factorizing}, rule
mining~\cite{mobasher2001effective,shao2009music,yap2012effective, yu2016dynamic}, Recurrent Neural Networks~\cite{liu2018stamp,wang2018attention,hidasi2015session}, and Convolutional Neural Networks~\cite{you2019hierarchical}.
  While they can model inter-item relations, they fall short in modeling intra-item semantics, especially when rich text data are available to represent the semantics of session items. 
  Furthermore, these
methods usually train models from scratch, which requires large amounts of
labeled data, especially when using complex models such as large neural
networks. (2) Large-scale pretrained language
models~\cite{lan2019albert,liu2019roberta,clark2020electra} have become
prevalent in natural language processing (NLP) tasks. Existing pretrained
learning models can serve as generic ``plug-in'' text encoders for text items, which can be then fine-tuned along with stacked neural modules for
session search and recommendation. However, while being effective to encode item semantics, pretrained language models are not designed to encode session graphs on items. Similar to our goal,
  several works that attempt to improve language models with graph-structured knowledge, such as in \cite{liu2020k,yao2019kg,shen2020exploiting}, where triplet relations extracted from knowledge graphs are learned to enrich the language models with knowledge base. 
  However, these models are only text encoders and cannot be used to jointly encode text items and session graphs. 


% \rui{revised statement: original: However, existing pretrained language
%   models are trained using generic text data, and have not taken intra-session
%   interactions between queries and products into consideration.} 

% \rui{our mdoel}

% \zc{This problem of this version is
%   that it is too brief. You need to describe what is the unique feature of your
%   method, and what are the benefits of your method. You need to keep this in
%   mind when writing later sections as well. For example, ``We propose a
%   pretrain model for semi-structured e-commerce session data, which can
%   serve as generic session encoders that simultaneously capture both intra-item
%   semantics and inter-item relations.''}.

We propose a pretrained model named \modelname (\modelfullname) for
semi-structured e-commerce session data, which can serve as a generic session
encoder that simultaneously captures both intra-item semantics and inter-item
relations. Different from existing pretrained models that can learn
representations of text or graph data, our model can learn representations of
text-based items as well as the relational session graphs that are built on
these items. Our model achieves this goal by performing the following two
pretrain tasks over unlabeled session data: (1) \textit{Intra-item
  masked language modeling}. This task requires the pretrained model to
predict masked tokens in session items from contextual text embeddings of the
same item. The learning of this task makes the pretrained model capture
domain-specific language for e-commerce. (2) \textit{Inter-item conditioned
  masked language modeling}. This tasks requires the model to use session
context, including inter-item interactions and global session information to
predict masked tokens in session items. By doing so, the model is encouraged
to pick up useful session-level signals to infer information about items. The integration of these two
pretrain tasks requires the model to capture not only domain-specific
semantics for session items, but also high-order inter-item correlations from
their text clues. Moreover, as a pretrained model for generic sessions,
\modelname can be trained on unlabeled session data and is more data-efficient
than existing models for session-based downstream tasks.


% XXX \zc{here, you should talk about the nice properties of
%   having a generic session pretrain models, /e.g./: generic encoders,
%   trained on unlabeled data, data efficient for downstream tasks.}

% \zc{this is unclear, do you mean predicting the tokens in the current item,
%   conditioned on other items?}

% The model is trained with two tasks: 1)  

To complete the above pretrain tasks, our model architecture tightly
integrates two key components: (1) an Item Transformer encoder, which captures text
semantics of session items; and (2) a Graph Conditioned Transformer, which aggregates
and propagates item-item relations for cross-item prediction. The Item
Transformer encoder is designed as a large-scale transformer model, in order to leverage the
flexibility and expressivity of self-attention to produce \emph{intra-item token embeddings} for session items. The Graph-Conditioned Transformer has
two modules: (i) a graph neural network module, which takes as input pooled item
 embeddings and aggregates neighborhood information on them,
yielding session-level item embeddings; 
%Then, the session-level item
%embeddings are treated as latent tokens, and a cross-attention transformer
%conditions text embeddings on the session-level embeddings, producing
%\emph{session-conditioned text embeddings}. 
and (ii) a cross-attention Transformer that treats session-level item embeddings as latent
tokens and produces \emph{inter-item token embeddings} by conditioning on the 
session-level items. The inter-item token embeddings  are infused with session-level 
inter-item information, and can be used to predict item tokens with session context.
%This models the higher-level 
%interactions between queries and products, while existing session-based
%approaches serializes sessions as customer behavioral sequences, ignoring the
%higher-order structure in a session. 
As a result, \modelname models the higher-level interactions between items in a session,
whereas existing pretrained approaches can only serialize sessions as sequences,
ignoring the higher-order session structures.
Our model brings together the
representation power of transformers as well as the ability of graph neural
networks in modeling high-order relations of different session items. During
pretrain, the structural knowledge of session graphs can help enrich the
text representations, and the text semantics can help the model better
understand inter-item interactions.

% \zc{polish this paragraph}

% an
% transformer-based language encoder and a graph neural network (GNN) relation encoder. 

% Our model consists of two parts: a language encoder and a session encoder. To
% summarize, the language encoder

% \rui{advantage, it feels like contributions already; im not sure if another paragraph is needed at the end}


% to 
% As a language
% modeler, we are able to produce meaningful representations of queries and
% products from text data, which are informative to the semantics and properties
% of queries and products.

We perform experiments on three session-based tasks:  product search, query search, and entity linking. 
We compare with publicly available state-of-the-art language models as well as
domain-specific language models trained on alternative representations of
session data, including product information, query-product interaction pairs,
and serialized behavioral sequences. Our experiments show that CERES
outperforms strong baselines on various session-based tasks by large margins. The encoder of our pretrained model performs better than existing language models even without the session encoder, showing that pretraining with the session encoder enriches the semantic representation of text data with session information. 
The better utilization of session information enables better understanding of customer preferences, making our model able to learn with very scarce training examples. 

We summarize our contributions as follows.
\vspace{-0.02in}
\begin{enumerate}
\item To the best of our knowledge, \modelname is the first pretrained model
  proposed for semi-structured e-commerce session data. \modelname can
  effectively encode both e-commerce items and sessions, and support various
  session-based downstream tasks generically. Further, \modelname is
  data-efficient and can achieve strong performance even when fine-tuned with
  a small amount of data for the target task.
  

  % We are the first to unify text and graph data in an end-to-end pretrain framework.
    %Our model architecture design combined transformers and graph neural networks.
    %Our design of pretrain tasks encourage the model to optimize both language representations and graph representations.

    % \hide{
    % \rui{rewrite}
    % \rui{og statement: We are the first to unify text and graph data in an end-to-end pretrain framework.
    % Our model architecture design combined transformers and graph neural networks.
    % Our design of pretrain tasks encourage the model to optimize both language representations and graph representations.}
    % We are the first to unify text and graph data in an end-to-end
    % pretrain framework. Compared with existing methods that utilize text
    % and graph data in pretrain, our method is a generic encoder for both
    % texts and graphs that can encode general graph structures on text data.
    % Our design of pretrain tasks encourages \zc{grammar mistake} the model to optimize both language and graph representations. }
    
\item We propose a new graph-conditioned transformer model architecture
  tailored for semi-structure sessions. This model not only leverages the
  self-attention mechanism to capture intra-item semantics, but also a
  graph-based cross-attention mechanism to capture inter-item contexts. Pretrained
  \modelname 
  
  thus enjoys both expressivity and flexibility for
  encoding the text and graph aspects in the semi-structured session.

%   inter-item token embeddings are infused with session-level 
% inter-item information, and can be used to predict item tokens with session context.

  % for session items.
  
  % are the first to train on semi-structured data where graphs are built
  % on text data. Compared with existing approaches that enhances text
  % pretraining with knowledge graph triplets, we are able to jointly encode
  % text and arbitrary graph structure.
    

 % \rui{should this be in 2 or 3?}

\item We conducted extensive experiments for three session-related tasks on a
  large-scale e-commerce benchmark. The results show the superiority of
  \modelname over strong baselines, including mainstay pretrained language
  models and state-of-the-art deep session recommendation models.

  % that we trained from scratch with session data to optimize domain-specific performance.

\end{enumerate}

==> method.tex <==
\section{The CERES Method}


In this section we introduce CERES for pretraining on semi-structured e-commerce session data, which can serve as generic session encoders that simultaneously capture both intra-item and and inter-item semantics. 
%We propose a pretraining framework for session data. 
%The inputs to our model are sessions in online e-commerce platforms. Each session can be posed as a relational graph, where nodes are queries and products, and edges indicate typed relations between them. Nodes in the graph can be represented as text data.
%We start by giving a formal definition of the input to our model \zc{polish your
%sentences, they read so casual.}.
Finally, we introduce the pretraining objectives and how CERES is used for
downstream tasks. \zc{revise this overview paragraph to make it consistent with
  the rest}

\hide{
Specifically, we define sessions as a graph \(G=(\vertexset, \edgeset)\), where 
\(\vertexset=(\queryset, \productset)\) is partitioned into ordered query set \(\queryset\) and unordered product set \(\productset\). 
Queries \(\queryset=(q_1,\ldots,q_n)\) is indexed by the order of the customer's searches. 
Suppose that the set of possible relation types is \(\actionset\). We define \(\edgeset = (\edgeset_q\cup\edgeset_a\). \(edgeset_q\) is the set of bidirectional edges,
where \(\edgeset_a \subset \{(q, p, a), q\in\queryset, p\in\productset, a\in\actionset\}\) specifies the relations between actions and queries. 
\(\edgeset_q=\{(q_i, q_j), i<j\}\) are one-directional connecting every query to its previous queries.
As such, each query has access to previous queries and products that were viewed or purchased under this query. 
}
\hide{
Specifically, we define sessions as a graph \(G=(\vertexset, \edgeset)\). Nodes
in the graph can be partitioned into two kinds of objects:
\(\vertexset=\queryset\cup \productset\) where \(\queryset\) is the query set
and \(\productset\) is the product set. Objects in the graph \(v\in \vertexset\)
can be represented as texts: \(v=(v_1,v_2,\ldots)\),  where \(v_i\)'s are sequence of tokens. 
}

% As in Section~\ref{sec:prelim}, we treat sessions as relational graphs, in which objects are text data. 
% Existing works are efficient to learn text data and graph data representations separately. However, the key challenge of our work is to 1) align the representation of underlying text data and higher level relational graph, and 2) compose higher level graph information given objects in the graph. \rui{challenges needs to be rewritten}

%To do so, the representation of text data is conditioned on the high level relations between objects. 
%A conditioned mask language modeling task ensures that graph information is efficiently utilized in the language modeling process. 
%As a result, the model is provided training signal to learn efficient representations of text and graphs and how to effectively utilize graph information to help language modeling.

\subsection{Session Pretraining Tasks}

\zc{This subsection is very important as it is unique to your method. It should
  occupy almost one page. Make it more detailed, add a figure, add
  mathematical formulation to make it appear more principled. Refer to the ElMo
  paper section 3.1-3.3. https://arxiv.org/pdf/1802.05365.pdf}
Generally, our model is pretrained on masked language modeling (MLM), which is a fill-in-the-blank task where the model is asked to fill in masked tokens by contextual information. We propose two MLM tasks: 1) \emph{intra-item masked language modeling}, which uses item-level context to predict masked tokens in queries and products; and 2) \emph{inter-level conditioned masked language modeling}, which uses session-level inter-item information to predict masked tokens.
By the first task, we ensure that the language encoder captures the text semantics in queries and products. The second task ensures that the session encoder can capture meaningful session-level information that is helpful for inferring item-level information.

\subsubsection{Masking Strategies}
\label{sec:masking_strat}
In this step, we introduce strategies for mask tokens in query and product texts.
To mask tokens in query texts, we follow the masking strategy of BERT~\cite{devlin2018bert}, where 15\% tokens are corrupted, in which the corrputed tokens are 1) replaced with \texttt{[MASK]} token 80\% of the time, 2) a random token 10\% of the time, and 3) unchanged 10\% of the time. 

For each product, as have a product sequence that consists of title and description, and a table of other attributes. 
The product sequence is masked in the same way as queries, i.e. with 15\% masked tokens. 
For other product attributes, because they are mostly short phrases or words, 
we employ an attribute-level masking strategy to ensure that the model is asked to predict product attribute information.
Specifically, 
for each of the other attribtues, there is a 50\% chance that this attribute is selected for masking.
If selected, 50\% tokens in the language descriptors of the attribute will be corrupted in the same way as masked tokens in queries are. It is always ensured that at least one token in the attribute is selected for masking.

\subsubsection{Loss Function}

To joinly optimize our model's representation ability for text and session
graph, the final loss function in the pretraining stage is the combination of
intra-item and inter-item masked language modeling loss. 
Specifically, intra-item MLM attaches a classification head after the language encoder to predict 
masked tokens in queries and products using context information in a single query or product itself.
Inter-item MLM attaches a classification head after the conditional transformer module
to predict masked tokens with session-level information as well. 

\subsection{Model Architecture}
To summarize, our model consists of two parts: 1) a langauge encoder, and 2) a
session encoder.
\zc{do not write it in
  this way, it is too plain and feels like you are simply concatenating existing
  stuff together. You should emphasize more on the unique aspect, /e.g./,
  graph-conditioned transformer}
The language encoder learns embeddings of queries and products in sessions from text semantics. 
The session encoder aggregates and propagates session information to query and product embeddings by \emph{graph-conditioned cross-attention}. \rui{term use "graph conditioned cross-attention, make sure of consistency in intro}
In the following sections we introduce the two parts respectively.

\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{assets/session_model_illustration.pdf}
  \caption{Illustration of our model framework \zc{delete framework}. Our model first encodes text data with a backbone transformer model, obtaining transformer output embeddings. Then the GNN model takes as input the session graph and the output embeddings as hidden states to output session-level node embeddings for each object in the session graph, which is encoded both text information and session information. Then, the object embeddings are conditioned on the session-level node embeddings to produce the final output embeddings conditioned on session information. }
  \label{fig:model_framework}
\end{figure}
\subsubsection{Transformer-Based Item Encoder}
\label{sec:transformers}
\zc{do not call it language encoder, be more problem-specific.}
We use self-attention based transformers~\cite{vaswani2017attention} to encode items in sessions, which can effectively capture the semantics encoded in their natural language descriptors. Compared with traditional representation learning on e-commerce data that rely on user-item interactions, our approach captures the linguistic prior in items that can reflect the semantic similarity between items. 
In this section we first introduce transformer models that are commonly used in modeling text data efficiently, including self-attention mechanisms and the composition of a transformer block. Then, we introduce how to use the transformer model to encode items in a session graph. In our setting, items could be either customer generated queries or products. We will introduce how to encode them separately. 

\paragraph{Transformer Model}
Transformers are the state-of-the-art model building blocks in natural language processing due to their accuracy, representation ability and efficiency in parallel computing that enabled large-scale pretraining and computations that previous recurrent neural network based models were hard to achieve. 
The commonly used transformer models consists of stacks of transformer blocks
that are based on self-attention modules. We introduce the transformers used in
this paper in the following section. \zc{do not write it like this, it still
  feels you are introducing others' work that have already been done. You should
revolve your method around the problem YOU are trying to solve. So you should
move the ``encoding session items, queries, products'' parts upfront here. The
logic flow will be like: queries and products are two major types of items in
e-commerce sessions, it will be important to capture the semantics in such
domain-specific text -> we choose to use transformer to encode the text, due to
the success of transformers and the expressive power of self-attention -> we
encode them like this (the equations for queries and products) -> in both
encoders, we use multi-head self-attention module to capture the contextual
semantics, like this (show the equations for multi-head self attention). Do not
use general notations like H and W, Q, K, V, but should be more problem-specific (/e.g./,
notations for queries)}

\paragraph{Multi-head Self-Attention.}
A multi-head self-attention layer is as described in \cite{vaswani2017attention}. Specifically, suppose that the input to the self-attention block is \(\mathbf{H}\in\mathbb{R}^{b\times d}\), the hidden size is \(d\) and the number of attention heads is \(h\), where it is always assumed \(h|d\), and \(d_h = h/d\). For each attention head, the input is linearly transformed to three matrices, \([\mathbf{Q}^i, \mathbf{K}^i, \mathbf{V}^i] = \mathbf{H}\mathbf{W}^i\) as queries, keys, and values, where \(\mathbf{W}^i\) is a \(d\times d_h\) weight matrix. The output of the \(i\)th attention head is
\begin{equation}
    \mathbf{O}^i = \mathrm{SelfAttention(\mathbf{H})} = \softmax(\frac{\mathbf{Q}^i(\mathbf{K}^i)^T}{\sqrt{d_h}})\mathbf{V}^i
    \label{eqn:attention}
\end{equation}
The output of the multihead attention is the concatenation of all heads output,
\begin{equation}
    \mathrm{MultiheadSelfAttention}(\mathbf{H}) = [\mathbf{O}^1,\ldots, \mathbf{O}^h]\in\mathbb{R}^{b\times d}
    \label{eqn:multiattention}
\end{equation}

\hide{
\paragraph{Transformer Blocks.} 
In this paper, we follow the transformer block design in Megatron-LM~\cite{shoeybi2019megatron}. Specifically, given input representations, 
}
\hide{
\paragraph{Transformer Block}
\begin{figure}
    \centering
    \includegraphics[width=0.35\linewidth]{assets/transformer_block.pdf}
    \caption{Transformer Block. \zc{terrible figure} this is just a waste of
      space. You waste the space to show how standard transformers do. You
      should use the space to show YOUR model.}
    \label{fig:transformer_block}
\end{figure}
}
%The computation of a transformer block is visualized in Figure~\ref{fig:transformer_block}. It consists of two parts: a multihead attention block and a MLP block. In both blocks, the inputs are first layer normalized, and then applied multihead attention and two-layer MLP with GeLU activation respectively, followed by dropout and residual connections. 
\paragraph{Encoding Session Items}
In this section we introduce how to use the transformers to encode items (queries and products) in sessions. 

\paragraph{Encoding Queries}
Each query \(q=[q_1,\ldots, q_n]\) is a sequence of tokens generated by customers as search keywords. 
We add a special token at the beginning of the queries, \texttt{[SEARCH]}, to indicate that the sequence represents a customer's search action.

We use the backbone transformer module
to obtain the token-level embedding of the queries and the pooled query
embedding by taking the embedding of the special token \texttt{[SEARCH]}: 
\begin{eqnarray}
   [\bq_1,\ldots,\bq_n] & = & \transformer([q_1,\ldots, q_n]) \nonumber \\
\bq & = & \ftpool([\bq_1,\ldots,\bq_n]) = \bq_1\nonumber
\end{eqnarray}
where \ftpool takes the first special token as the pooling of a sequence of embeddings, \(\bq_1,\ldots, \bq_n\) are query token embeddings, and \(\bq\) the pooled query embedding.

\paragraph{Encoding Products}
\hide{
Each product \(p\) is a table of product titles, product descriptions and \(K\) attributes: \(p_1,\ldots, p_K\), each having an attribute type and text sequence: \([p_{i1}, p_{i2}, \ldots], i=1,\ldots, K\).
We concatenate the product title and potential bullets as the product sequence \(p=[p_{01}, p_{02}, \ldots]\), with special tokens \texttt{[TITLE]} and \texttt{[BULLET]} in front of of them respectively.
Like in encoding queries, we pass them through the transformer to obtain token embeddings \([\bp_{01}, \bp_{02}, \ldots]\) and pooled embedding \([bp_0]\).

The other attribute types are processed likewise. Specifically, they are added special tokens at the beginning of the attribute sequences that represent their attribute types. The final pooled embedding of product \(\bp\) is the average of the embeddings of all attributes, including the pooled product sequence. 
}
Each product \(p\) is a table of \(K\) attributes: \(p_1,\ldots, p_K\), where \(p_1\) is always the \emph{product sequence}, which is the concatenation of product title and description. 
Each attribute \(p_i=[p_{i1}, p_{i2}, \ldots]\) starts with a special token \([\texttt{ATTRTYPE}]\), where \texttt{ATTRTYPE} is replaced with the language descriptor of the attribtue. 
Then, the transformer is used to capture attribute semantics:
 \rui{This would be essentially the same as the previous equations; would it be necessary to rewrite them?}
\begin{equation}
    \begin{aligned}
   \ [\bp_{i1}, \bp_{i2}, \ldots] & = \transformer([p_{i1}, p_{i2}, \ldots] \nonumber \\
\bp_i & = \ftpool([\bp_{i1}, \bp_{i2}, \ldots] , i=1,\ldots, K\nonumber \\
\bp & = \avgpool([\bp_1,\ldots,\bp_k])
\end{aligned}
\end{equation}
where \(\bp_i\) are attribute embeddings, and \avgpool takes average pooling of attribute embeddings for product embedding. 
\zc{after encoding, you should tell readers what is this encoding for. For
  example, it can be used for intra-item pre-training task. And it will also be
  plugged into the session encoder for inter-item pre-training task.}

\subsubsection{Session Encoder}
\zc{Graph-Conditioned Transformer for Session Encoding}
In the above, we introduced how to obtain session item embeddings by modeling with transformer their unstructured text descriptors. So far, these embeddings only capture intra-item semantics and are unaware of session-level information or inter-item interactions. 

In the following section, we put session items in a structured session context to infuse session-level inter-item information in items embeddings. 
To achieve this, we use graph attention modules to obtain item-level session embeddings that encode the session information centered on given items. These embeddings will play a vital role in the next session for modeling text data conditioned on session information. First, we introduce graph attention modules.

\paragraph{Graph Attention Modules}

In this paper, we adopt graph attention modules, \zc{again do not write it like
  this. You waste your precious space, and leave the impression that you are
  just using an existing GNN model. Describe your method around your problem.
  Like: session data are semi-structured, it is important for the pre-training
  model to capture the dependencies/relations between items. -> we design
a graph-conditioned transformer for capturing relations and the
inter-item pre-training task. -> this module uses graph neural network to
propagate the embeddings, and then use anther transformer layer to aggregate the context.
} where we use multihead
attention similar to the method introduced in Section\ref{sec:transformers} to
aggregate neighborhood information for each node.
The attention computation in \eqref{eqn:attention} and \eqref{eqn:multiattention} is equivalent to updating vertices in a \(b\)-complete graph. The defining difference in graph neural network layers is that we assume an adjacency matrix as a filter to where vertices may attend to as neighbors:
\begin{equation}
    \mathrm{GraphAttention}(\mathbf{H}, \mathbf{A}) = \softmax(\frac{\mathbf{Q}^i(\mathbf{K}^i)^T}{\sqrt{d_h}}) \mathbf{A} \mathbf{V}^i 
    \label{eqn:attention}
\end{equation}
where \(\mathbf{A}\) is a \(b\times b\) adjacency matrix. The rest of the computation is the same as the previously defined transformer block. 

\paragraph{Modeling Session Graph Relations via GAT}
After encoding products and queries, they are treated as vertices in the session graph: \((\bq_1,\ldots, \bq_N, \bp_1,\ldots, \bp_M)\). As queries are sequential in nature, we train a query positional embedding and add them to the query embeddings. 

A graph neural network module that consists of graph neural network blocks are used to infuse vertex embeddings with session information. Specifically, we build an adjacency matrix \(\mathbf{A}\) encodes the relations between queries and vertices as introduced in Section~\ref{sec:session_graph}. Then, the product and query embeddings are treated as vertex hidden states and fed to the graph neural network blocks with the adjacency matrix. The output of the graph neural network module updates product and query embeddings with session information:
\begin{equation}
    [\bq_1^s,\ldots, \bq_n^s, \bp_1^s,\ldots, \bp_m^s] = \mathrm{GNN}([\bq_1,\ldots, \bq_n, \bp_1,\ldots, \bp_m], \mathbf{A}) 
\end{equation}
where \([\bq_1^s,\ldots, \bq_n^s, \bp_1^s,\ldots, \bp_m^s]\) are now session-level query and product embeddings. 

\paragraph{Conditional Text Data Modeling}
In this stage, another sequence of transformer blocks are built and used to obtain sequence embeddings conditioned on session graph information. We call the said transformer the \emph{conditional transformer module}.
 Specifically, 
we take the output token embeddings of the query and product encoders as input.
\zc{do not just plainly write how you do. You should SELL, and justify why you
  want to do this.} But at this time, we want them to be conditioned on their neighbors in the session graph. 
For a query or product, say \(v\), we represent its neighborhood by the average embedding of all its neighbors:
\begin{equation}
     \overline{\mathcal{N}(\mathbf{v})} = \frac{1}{|\mathcal{N}(v)|}\sum_{u\in \mathcal{N}(v)} \mathbf{u}
\end{equation}
Then we use a 3-layer MLP \zc{the writing style is too dry, not interesting at all.} to map the neighborhood embedding to D latent spaces:
\begin{equation}
    [\bc_1,\ldots, \bc_D] = \mathrm{MLP}(\overline{\mathcal{N}(\mathbf{v})})
\end{equation}
We treat these \(D\) embeddings as implicit conditional tokens before the query or product \(v\). Hence, the conditional language model takes the following sequence as input:
\begin{equation}
    [\bc_1,\ldots, \bc_D, [\mathrm{BOS}], \bv_1,\ldots, \bv_n]
\end{equation}
where \texttt{[BOS]} is the special token signifying the type of \(v\). \zc{what
is bold c u v?} For queries, it is \texttt{[SEARCH]}, where as for product attributes it is the name of the attribute. 
The conditioned sequence is passed through a 2-layer self-attention-based Transformer, yielding final token embeddings and query/product embeddings conditioned on session information.

\subsection{Finetuning for Downstream Tasks}
\label{sec:finetuning}
\rui{Im not sure if to remove this section and merge it with the following sections introducing downstream tasks.}
We use the same retrieval head for all tasks. To summarize, we encode sessions and the retrieve items separately, and compare the cosine similarities between sessions and objects for ranking and predictions. 

\subsubsection{Encoding Sessions}
To encode sessions with a given pretrained model in the finetuning stage, we
first encode objects in sessions and obtain their embeddings. For Congrats, the
embedding outputs at this point are conditioned on session information, while
for other baseline models, the objects are independently encoded.  \zc{clearly,
  this needs to be revised to fit into this section, not the previous version of
your experiments.}
Then, we take the average pooling of all objects in a session as the session embedding.

\subsubsection{Loss function}
Suppose that we've obtained session and item embeddings. To measure the relevance of an item to a given session, we first transform the obtained embeddings by separate linear layers. Denote the transformed session embeddings as \(\mathbf{s}\) and item embeddings as \(\mathbf{y}\). 
The similarity between them is computed by cosine similarity \(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y})\). 
To finetune the models and the additional linear weights, we optimize the following hinge loss:

\begin{equation}
    \ell_{\mathbf{finetune}} = (\max(\epsilon^+ - \mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}), 0))^2 + (\max(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}^-), 0)-\epsilon^-, 0))^2
\end{equation}
where \(y^-\) is a uniformly sampled negative item. 
For each positive item, we'll sample 5 negative samples to compute the hinge loss. We choose \(\epsilon^+=0.9\) and \(\epsilon^-=0.2\). 

\zc{can you add a baseline of graph
  neural network?}


% \reminder{Domain-specific Phrase Sampling Here}


% \subsubsection{Contrastive Learning}

% 1. Query - next query prediction. 
% 2. Query2Product - sample negative products for constrastive learning. 


==> method_new__Zhang_Chao_s_conflicted_copy_2022-01-15_.tex <==
\section{The CERES Method}

In this section we introduce the details of CERES. We first describe our
designed session pretraining task in Section~\ref{sec:glmm}, and then describe
the model architecture of CERES in Section \ref{sect:model}. We illustrate our model architecture in Figure~\ref{fig:model_illustration}.

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{assets/framework.pdf}
    \caption{Model illustration. CERES first produces intra-item embeddings in the Item Transformer Encoder. Then, the Graph-Conditioned Transformer aggregates and propagates session-level information to obtain inter-item embeddings. }
    \label{fig:model_illustration}
\end{figure*}

% including how to encode different types of session items, model architecture, and how to mask tokens for graph-conditioned masked language modeling introduced .
\vspace{-0.1in}
\subsection{Graph-Conditioned Masked Language Model}
\label{sec:glmm}
Suppose \(\mathcal{G}=(\mathcal{V}, \mathcal{E})\) is a graph on \(T\) text items as vertices, \(v_1,\ldots, v_T\), each of which is a sequence of text tokens: \(v_i=[v_{i1},\ldots,v_{iT_i}]\), \(i=1,\ldots, T\). 
We propose \emph{graph-conditioned masked language modeling} (GMLM), where masked tokens are predicted with both intra-item context and inter-item context:
\begin{equation}
\small
    p_{\textrm{GMLM}}(v_{\textrm{masked}}) = \prod_{j\textrm{th\ masked}} \mathbb{P}(v_{ij} |  \mathcal{G}, \{v_{ik}\}_{k\textrm{th\ unmasked}}),
    \label{eqn:gmlm}
\end{equation}
which encourages the model to leverage information graph-level inter-item semantics efficiently in order to predict masked tokens. To optimize \eqref{eqn:gmlm}, we need to learn token-level embeddings that are infused with session-level information, which we introduce in Section~\ref{sec:cond_transformer}. Suppose certain tokens in the input
sequence of items are masked (detailed below), we optimize the predictions of the
masked tokens with cross entropy loss.

\hide{
Compared with Equation MLM, the graph-level inter-item semantics are
also used to predict masked tokens. Equation \eqref{eqn:gmlm} thus encourages
the model to not only learn good semantic representations of text, but also how
to utilize inter-item relations to predict information within an item. To
optimize Equation \eqref{eqn:gmlm}, %we can build a token prediction head on top
%of \([v_{i1}^c, \ldots, v_{iN_i}^c]\) \rui{reminder to explain this embedding} . Suppose certain tokens in the input
we need to learn token-level embeddings that are infused with session-level and inter-item information, which we introduce in Section~\ref{sec:cond_transformer}. Suppose certain tokens in the input
sequence of items as masked (detailed below), we optimize the predictions of the
masked tokens with cross entropy loss. }
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{assets/pretraining.pdf}
    \caption{Pretraining framework illustration. CERES learns both inter-item and intra-item embeddings for item tokens for Masked LM and Graph-Conditioned Masked LM. In practice, we find it beneficial to optimize both.}
    \label{fig:pretraining}
\end{figure}

\vpara{Token Masking Strategy.} \hide{During pretraining, we mask tokens from queries
and products in a session.
To mask tokens in query texts, we follow the masking strategy of BERT~\cite{devlin2018bert}, where 15\% tokens are corrupted, in which the corrputed tokens are 1) replaced with \texttt{[MASK]} token 80\% of the time, 2) a random token 10\% of the time, and 3) unchanged 10\% of the time. 

For each product, we have a product sequence that consists of its title and description, and a table of other attributes. 
The product sequence is masked in the same way as queries, \textit{i.e.}, with 15\% masked tokens. 
For other product attributes, because they are mostly short phrases or words, 
we employ an attribute-level masking strategy to ensure that the model is asked to predict product attribute information.
Specifically, 
for each of the other attribtues, there is a 50\% chance that this attribute is selected for masking.
If selected, 50\% tokens in the language descriptors of the attribute will be corrupted in the same way as masked tokens in queries are. It is always ensured that at least one token in the attribute is selected for masking.}
To mask tokens in long sequences, including product titles and descriptions, we follow~\cite{devlin2018bert} and choose 15\% of the tokens for masking. For short sequences, including queries and product attributes, there is a 50\% probability that a short sequence will be masked, and for those sequences 50\% of their tokens are selected for masking. 
%The masked tokens are processed according to ~\cite{devlin2018bert}, \textit{i.e.} 1) replaced with \texttt{[MASK]} token 80\% of the time, 2) a random token 10\% of the time, and 3) unchanged 10\% of the time.


% \rui{I put a paragraph here to explain why we need to design such a model. }
%In order to compute ~\eqref{eqn:gmlm}, a model needs to compute token embeddings that have access to session-level information, on which the model can predict a distribution over the vocabulary. 
%To facilitate this, we design a \emph{Graph-Conditioned Transformer for Session Encoding} that can effectively infuse session-level inter-item information in token-level intra-item information.  
%Specifically, we use a \emph{Transformer-based Session Item Encoder} to first encode all items in a session: 
\vspace{-0.1in}

\subsection{Model Architecture}
\label{sect:model}

%To effectively model token probability in a session context, namely Equation
%~\eqref{eqn:gmlm}, 
To model the probability in ~\eqref{eqn:gmlm},
we design two key components in the CERES model: 1) a
\emph{Transformer-based Item Encoder}, which produces token-level intra-item
embeddings that contain context information within a single item; and 2)
a \emph{Graph-Conditioned Transformer for Session Encoding}, which produces
session-level embeddings that encodes inter-item relations, and propagates the
session-level information back to token-level. 

\subsubsection{Item Transformer Encoder}
\label{sec:item-encoder}

The session item encoder aims to encode intra-item textual information for each
item in a session. We design the item encoder based on Transformers, which allows
CERES to
leverage the expressive power of the self-attention mechanism for modeling
domain-specific language in e-commerce sessions.
Specifically, given an
item \(i\), the transformer-based item encoder compute its token embeddings as
follows: %\zc{better to add equations and stuff for multi-head self attention}:
\begin{equation}
\small
  \begin{aligned}
  \ [\bv_{i1}, \ldots, \bv_{iT_i}] & = \mathrm{Transformer}_{\mathrm{item}}([v_{i1}, \ldots, v_{iT_i}] ) \\
  \bv_{i} & = \mathrm{Pool}([v_{i1}, \ldots, v_{iT_i}]),
  \end{aligned}
  \label{eqn:uncond_embedding}
\end{equation}
where \(\bv_{ij}\) is the embedding of the \(j\)th token in the \(i\)th item, and \(\bv_i\) is the pooled embedding of the \(i\)th item.
At this stage, \(\{\bv_{ij}\}, \{\bv_i\}\) are embeddings that only encode the intra-item information. 

% In this section, we introduce how to compute token-level and item-level embeddings in Section~\ref{sec:item-encoder}.
% We use Transformer~\cite{vaswani2017attention} to encode text data in session items. Consistent with Section~\ref{sec:item-encoder}, we denote this Transformer as \(\mathrm{Transformer}_{\mathrm{item}}\).

\vpara{Details of Item Encoding.}
There are two types of items in a session: queries and products. We detail the
encoding procedures for these two item types below.

Each query \(q_i=[q_{i1},\ldots, q_{iT_i}]\) is a sequence of tokens generated by customers as search keywords. 
We add a special token at the beginning of the queries, \texttt{[SEARCH]}, to indicate that the sequence represents a customer's search keywords. 
Then, to obtain the token-level embedding of the queries and the pooled query
embedding by taking the embedding of the special token \texttt{[SEARCH]}.


Each product \(p_i\) is a table of \(K\) attributes: \(p^1,\ldots, p^K\), where \(p^1\) is always the \emph{product sequence}, which is the concatenation of product title and bullet description. 
Each attribute \(p_i^k=[p_{i1}^k, p_{i2}^k, \ldots]\) starts with a special token \([\texttt{ATTRTYPE}]\), where \texttt{ATTRTYPE} is replaced with the language descriptor of the attribtue. 
\hide{Then, the transformer is used to capture attribute semantics:
 % \rui{This would be essentially the same as the previous equations; would it be necessary to rewrite them?}
\begin{equation}
\small
    \begin{aligned}
   \ [\bp_{i1}^k, \bp_{i2}^k, \ldots] & = \transformer([p_{i1}^k, p_{i2}^k, \ldots]) \nonumber \\
\bp_i^k & = \ftpool([\bp_{i1}^k, \bp_{i2}^k, \ldots]) , k=1,\ldots, K\nonumber \\
\bp_i & = \avgpool([\bp_1^1,\ldots,\bp_i^K])
\end{aligned}
\end{equation}
where \(\bp_i^k\) is the \(k\)th attribute embedding for the \(i\)th product.}
Then, the Transformer is used to compute token and sentence embeddings for all attributes. The product embedding is obtained by average pooling of all attribute's sentence embeddings. 

\hide{
In existing application of Transformers~\cite{devlin2018bert,liu2019roberta,clark2020electra}, tokens embeddings are usually added with positional embeddings to encode the positional information of tokens in the text sequence.} 

\hide{
We also note that, existing
works~\cite{devlin2018bert,liu2019roberta,clark2020electra} employ a
\emph{positional embedding} which maps discrete integers to continuous vectors.
Tokens in the \(k\)th position are added with the \(k\)th positional embedding.
This encodes positional information of tokens in Transformers,
which are undirectional in nature \zc{This paragraph is confusing to me. How do
  you handle the directional nature of sessions? Simply by preserving 0? I
  expect you to describe something like: In contrast, the items in sessions are
  directional/ordered, the ext position encoding can cause XXX problem. We thus
  XXX. Revise this paragraph to make it stronger}. 
While existing works index tokens starting from \(0\) as is natural, we start
from \(1\) instead, reserving \(0\) for latent conditioning tokens.
}


\subsubsection{Graph-Conditioned Session Transformer}
\label{sec:cond_transformer}
%Thus far, we have described the transformed-based item encoder for capturing
%intra-item semantics. 
The Graph-Conditioned Session Transformer aims to infuse intra-item and
inter-item information to produce item and token embeddings. For this purpose,
we first design a \textit{position-aware graph neural network} (PGNN) to capture
the inter-item dependencies in a session graph to produce item embeddings. Then
conditioned on the PGNN-learned item embedding, we propose a cross-attention
Transformer, which produces infused item and token embeddings for the
Graph-Conditioned Masked Language Modeling task.

\vpara{Position-Aware Graph Neural Network.} We use a GNN to capture inter-item relations. This will allow CERES to obtain item embeddings that encode the
information from other locally correlated items in the session. Let $[\bv_{1},
\ldots, \bv_{N}]$ denote the item embeddings produced by the intra-item
transformer encoder. 
We treat them as hidden states of nodes in the session graph \(\mathcal{G}\) and feed them to the GNN model, obtaining session-level item embeddings \([{\bv}^h_{1}, \ldots, {\bv}^h_{N}]\). 
\hide{We use a graph neural network to infuse information from
other items in the session to produced pooled item embeddings:
\begin{equation}
\small
  [{\bv}^h_{1}, \ldots, {\bv}^h_{N}] = \mathrm{GNN}([\bv_{1}, \ldots, \bv_{N}], \mathcal{G}),
\end{equation}
which aggregates neighborhood information for each item in a session graph. Particularly, we use a multi-head attention
based Graph Attention Network~\cite{velivckovic2017graph} which learns a soft
selection of neighbors for each item to pool information from.}

The items in a session graph are sequential according to the order the customers generated them. To let the GNN model
learn of the positional information of items, we train an \emph{item
  positional embedding} in analogous to positional embedding of tokens. Before
feeding the item embeddings to GNN, the pooled item embeddings are added
item positional embeddings according to their positions in the session's item
sequence. In this way, the item embeddings \(\{\bv^i\}_{i\in\mathcal{V}}\)
are encoded their positional information as well.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{assets/cross-attention.pdf}
    \caption{Illustration of cross-attention over latent conditioning tokens. The item token embeddings perform self-attention as well as cross-attention over latent conditioning tokens, thus incorporating session-level information. Latent conditioning tokens perform self-attention to update their embeddings, but do not attend to item tokens to preserve session-level information. }
    \label{fig:cross-attention}
\end{figure}
\vpara{Cross-Attention Transformer.} Conditioned on PGNN, we design a
\textit{cross-attention transformer} which propagates session-level information in PGNN-produced item embeddings to all tokens to produce token embeddings that are infused with both intra-item and inter-item information. 

In order to propagate item embeddings to tokens, we treat item embeddings as
latent tokens that can be treated as a ``part'' of item texts. 
for each item \(i\), we first expand \(\bv_i^h\) to \(K\) latent conditioning tokens by using a multilayer perceptron module to map \(\bv_i^h\) to \(K\) embedding vectors \([\bv_{i1}^h,\ldots, \bv_{iK}^h]\) of the same size. 
For each item \(i\), we compute its latent conditioning tokens by averaging all latent tokens in its neighborhood.
Suppose \(N(i)\) is the set of all neighboring items in the session graph, itself included. In each position, we take the average of the latent token embeddings in \(N(i)\)
\hide{: 
\begin{equation}
    \begin{aligned}
    \overline{\bv}_{ik}^h = {|N(i)|}^{-1} \sum_{j\in N(i)} \bv_{jk}^h, k=1,\ldots, K,
    \end{aligned}
\end{equation}}
  
as the \(k\)th latent conditioning token, \(\overline{\bv}_{ik}^h\), for the \(i\)th item.
Then, we concatenate the latent conditioning token embeddings 
and the item token embeddings obtained by the session item encoder:
\begin{equation}
  [\overline{\bv}_{i1}^h,\ldots, \overline{\bv}_{iK}^h, \bv_{i1}, \ldots, \bv_{iN_i}].
\end{equation}
%This sequence of embeddings encode both the intra-item token level information in the original tokens \(\{\bv_{ij}\}_{j=1}^{N_i}\) and the inter-item session-level information in the latent conditioning tokens \(\{\overline{\bv}_{ik}^h\}_{k=1}^K\). 
\hide{
which encodes both the intra-item token level information in the original tokens \(\{\bv_{ij}\}_{j=1}^{N_i}\) and the inter-item session-level information in the latent conditioning tokens \(\{\overline{\bv}_{ik}^h\}_{k=1}^K\).
Then, we compute the token-level embeddings with session information:
\begin{equation}
\small
\begin{aligned}
  \ [\bv_{i1}^c, \ldots, \bv_{iN_i}^c] = \mathrm{Transformer}_{\mathrm{cond}}(([\overline{\bv}_{i1}^h,\ldots,  \overline{\bv}_{iK}^h, \\ \bv_{i1}, \ldots, \bv_{iN_i}]),
\end{aligned}
  \label{eqn:final_conditioned_embedding}
\end{equation}
where the Transformer module facilitates the cross-attention between original
tokens and latent conditioning tokens to produce
\(\{\bv_{ij}^c\}_{j=1}^{N_{i}}\). They are the token embeddings of the \(i\)-th
item infused with both item-level and session-level information. }
Then, we compute the token-level embeddings with session information by feeding the concatenated sequence to a shallow cross-attention Transformer.

 The cross-attention
Transformer is of the same structure as normal Transformers. \hide{The difference is in the attention
mechanism where in cross-attention Transformer, 1) original item tokens perform
self-attention over themselves; 2) latent conditioning tokens perform
self-attention over themselves; and 3) original item tokens perform
cross-attention over latent conditioning tokens. Particularly, latent
conditioning tokens do not have access to original tokens to prevent the influx
of intra-item information potentially diluating session-level information stored
in latent conditioning tokens. Illustration of cross-attention Transformer is provided in Figrue~\ref{fig:cross-attention}.}
The difference is that we prohibit the latent conditioning tokens from attending over original item tokens to prevent the influx
of intra-item information potentially diluating session-level information stored
in latent conditioning tokens. Illustration of cross-attention Transformer is provided in Figrue~\ref{fig:cross-attention}.

We use the embeddings produced by this cross-attention Transformer as the final
embeddings for modeling the token probabilities in Equation \eqref{eqn:gmlm} and
learning the masked language modeling tasks. During training, the model is
encouraged to learn good token embeddings with the Item Transformer Encoder, as
better embeddings \(\{{\bv_{ij}}\}_{j=1}^{N_i}\) is necessary to improve the
quality of \(\{{\bv^c_{ij}}\}_{j=1}^{N_i}\). \hide{The GNN module in the session
transformer will be encouraged produce more effective session-level embeddings
to be infused in token embeddings by the Transformer for optimization of the
cross entropy loss \zc{this sentence is unclear}.} The Graph-Conditioned Transformer will be encouraged to produce high-quality session-level embeddings for the GMLM task. Hence, CERES is encouraged to
produce high-quality embeddings that unify both intra-item and
inter-item information.
\vspace{-0.1in}
\subsection{Finetuning}
\label{sec:finetuning}
When finetuning CERES for downstream tasks, 
we first obtain session-level item embeddings. The session embedding is computed as the average of all item embeddings. To obtain embedding for a single item without session context, such as for retrieved items in recommendation tasks, only the Item Transformer Encoder is used. 

To measure the relevance of an item to a given session, we first transform the obtained embeddings by separate linear maps. Denote the transformed session embeddings as \(\mathbf{s}\) and item embeddings as \(\mathbf{y}\). 
The similarity between them is computed by cosine similarity \(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y})\). 
\hide{To finetune the models and the additional linear weights, we optimize the following hinge loss:
\begin{equation}
\begin{aligned}
    \ell_{\mathbf{finetune}} & = (\max(\epsilon^+ - \mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}), 0))^2 \\ & + (\max(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}^-), 0)-\epsilon^-, 0))^2
\end{aligned}
\end{equation}
where \(y^-\) is a uniformly sampled negative item. 
For each positive item, we'll sample 5 negative samples to compute the hinge loss. We choose \(\epsilon^+=0.9\) and \(\epsilon^-=0.2\). }
To finetune the model, we optimize a hinge loss on the cosine similarity between sessions and items.

\hide{
\subsection{Finetuning}
\label{sec:finetuning}
We use the same retrieval head for all tasks. To summarize, we encode sessions and the retrieve items separately, and compare the cosine similarities between sessions and objects for ranking and predictions. 

\subsubsection{Encoding Sessions}
To encode sessions with a given pretrained model in the finetuning stage, we
first encode objects in sessions and obtain their embeddings. For Congrats, the
embedding outputs at this point are conditioned on session information, while
for other baseline models, the objects are independently encoded.  \zc{clearly,
  this needs to be revised to fit into this section, not the previous version of
your experiments.}
Then, we take the average pooling of all objects in a session as the session embedding.

\subsubsection{Loss function}
Suppose that we've obtained session and item embeddings. To measure the relevance of an item to a given session, we first transform the obtained embeddings by separate linear layers. Denote the transformed session embeddings as \(\mathbf{s}\) and item embeddings as \(\mathbf{y}\). 
The similarity between them is computed by cosine similarity \(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y})\). 
To finetune the models and the additional linear weights, we optimize the following hinge loss:

\begin{equation}
    \ell_{\mathbf{finetune}} = (\max(\epsilon^+ - \mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}), 0))^2 + (\max(\mathrm{d}_\mathbf{cos} (\mathbf{s}, \mathbf{y}^-), 0)-\epsilon^-, 0))^2
\end{equation}
where \(y^-\) is a uniformly sampled negative item. 
For each positive item, we'll sample 5 negative samples to compute the hinge loss. We choose \(\epsilon^+=0.9\) and \(\epsilon^-=0.2\). 

\}}




% \hide{
% \subsection{Model Architecture.}
% CERES adopts a hidden size of 768 across all modules. The \(\mathrm{Transformer}_\mathrm{item}\) in the Session-item Transformer Encoder uses a 12-layer Transformer the same as ~\cite{shoeybi2019megatron}. In the Graph-Conditioned Session Transformer, for the \(\mathrm{GNN}\), we use a 2-layer Graph Attention Network~\cite{vaswani2017attention}, where an attention block is defined the same as in ~\cite{shoeybi2019megatron}, except that self-attention is replaced with graph-based attention. For \(\mathrm{Transformer}_\mathrm{cond}\), a 3-layer Transformer with the same structure as ~\cite{shoeybi2019megatron} is used. 
% }


==> model_new.tex <==
\section{Our Method}
In this section we introduce our method. 

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{assets/framework.pdf}
    \caption{Rough Framework}
    \label{fig:model_framework}
\end{figure*}

\subsection{Model Input}

The input to our model are graphs with customer generated queries and products as vertices. Specifically, a session \(\session=(\queryset, \productset, \edgeset)\) is a collection of ordered query set \(\queryset=[q_1,\ldots, q_n]\), and ordered product set \(\productset=[p_1, \ldots, p_n]\). 
The edge set \(\edgeset\) contains the connections between queries and products and among queries themselves.

We propose a \reminder{model name}\modelname to capture the structural and linguistic information within a session. 


\subsection{Backbone Linguistic Encoder}
The fundamental of our model is a backbone linguistic encoder. Following previous works, we employ a BERT-like model structure to encode linguistic objects in our model. 


\subsubsection{Encoding Queries}
The first steps of our framework encode nodes in the session graph, i.e. queries products.
In the query set \(\queryset\), each query \(q_i\) is a sequence of tokens generated by the customer to prompt the search engine. 
We add a special token at the beginning of the queries, \texttt{[SEARCH]}, to indicate that the sequence represents a customer's search action.

We use a BERT-like Transformer encoder to obtain the token-level embedding of the queries and the pooled query embedding by taking the embedding of the special token \texttt{[SEARCH]}. We use bold superscripted letters \(\bq_i^1, \bq_i^2, \ldots\) to denote the the token embeddings of the \(i\)th query, and bold letters without superscripts \(\bq_i\) to denote the pooled embedding of the query.

\subsubsection{Encoding Products}
Each product \(p_i\in\productset\) is a table of \(K\) attributes: \(p_{i1},\ldots, p_{iK}\). Each attribute \(p_{iK}\) has an attribute type and a sequence of tokens. In particular, each product is guaranteed to have a product title and bullet description. 

Like in encoding queries, we add a special token \texttt{[ATTR\_TYPE]}, where \texttt{ATTR\_TYPE} is the name of the attribute type, before the tokens of the attribute and pass them through the BERT-like Transformer. 
Each attribute has a pooled embedding \(\bp_{ik}\). We take the average of the attribute embeddings as the product embedding. 

\subsubsection{Modeling Session Graph Relations via GAT}

After we have the embeddings of queries and products in the session graph, we pass them through a Graph Attention Network to aggregate neighborhood information. After this operation, the embeddings of queries and products will be encoded contextual information in a session. 

To make sure that the model has access to the order information of queries, we add the query embeddings with query position embedding. 


\subsubsection{Conditional Language Modeling Layers}
In this stage, we perform a conditional langauge modeling by a BERT-like Transformer. Specifically, 
we take the output token embeddings of the query and product encoders as input. But at this time, we want them to be conditioned on their neighbors in the session graph. 
For a query or product, say \(v\), we represent its neighborhood by the average embedding of all its neighbors:
\begin{equation}
     \overline{\mathcal{N}(\mathbf{v})} = \frac{1}{|\mathcal{N}(v)|}\sum_{u\in \mathcal{N}(v)} \mathbf{u}
\end{equation}
Then we use a 3-layer MLP to map the neighborhood embedding to D latent spaces:
\begin{equation}
    [\bc_1,\ldots, \bc_D] = \mathrm{MLP}(\overline{\mathcal{N}(\mathbf{v})})
\end{equation}
We treat these \(D\) embeddings as implicit conditional tokens before the query or product \(v\). Hence, the conditional language model takes the following sequence as input:
\begin{equation}
    [\bc_1,\ldots, \bc_D, [\mathrm{BOS}], \bv_1,\ldots, \bv_n]
\end{equation}
where \texttt{[BOS]} is the special token signifying the type of \(v\). For queries, it is \texttt{[SEARCH]}, where as for product attributes it is the name of the attribute. 
The conditioned sequence is passed through a 2-layer self-attention-based Transformer, yielding final token embeddings and query/product embeddings conditioned on session information. 

\subsubsection{Masked Language Modeling}

% \reminder{Domain-specific Phrase Sampling Here}


% \subsubsection{Contrastive Learning}

% 1. Query - next query prediction. 
% 2. Query2Product - sample negative products for constrastive learning. 

